Minerva: A File-Based Ransomware Detector

Ransomware attacks have caused billions of dollars in damages in recent years, and are expected to cause billions more in the future. Consequently, significant effort has been devoted to ransomware detection and mitigation. Behavioral-based ransomware detection approaches have garnered considerable attention recently. These behavioral detectors typically rely on process-based behavioral profiles to identify malicious behaviors. However, with an increasing body of literature highlighting the vulnerability of such approaches to evasion attacks, a comprehensive solution to the ransomware problem remains elusive. This paper presents Minerva, a novel, robust approach to ransomware detection. Minerva is engineered to be robust by design against evasion attacks, with architectural and feature selection choices informed by their resilience to adversarial manipulation. We conduct a comprehensive analysis of Minerva across a diverse spectrum of ransomware types, encompassing unseen ransomware as well as variants designed specifically to evade Minerva. Our evaluation showcases the ability of Minerva to accurately identify ransomware, generalize to unseen threats, and withstand evasion attacks. Furthermore, over 99% of detected ransomware are identified within 0.52sec of activity, enabling the adoption of data loss prevention techniques with near-zero overhead.

==> sections/07-related_work.tex <==
\section{Related Work}\label{sec:related}

Process-based behavioral ransomware detection~\cite{kirda_unveil,kirda_redemption,scaife_cryptolock_2016,continella_shieldfs:_2016,mehnaz_rwguard,de_gaspari_evading_2022} attempts to identify running ransomware processes by analyzing features derived from their execution.
Beyond ransomware, many dynamic malware detection techniques have been proposed based on analyzing system calls and other dynamic characteristics~\cite{ye_survey_2017}.
Several approaches focus on using high entropy as a proxy to detect ransomware encryption activity. These approaches use various techniques, including $\chi^2$-test~\cite{lipmaa_data_2017} and the Kullback-Liebler divergence~\cite{foresti_efficient_2016}. As we discussed earlier, in isolation, entropy is a weak distinguisher of ransomware activity and can be easily evaded~\cite{de_gaspari_reliable_2022}.

Another line of work utilizes decoy files~\cite{genc_deception_2019,moore_detecting_2016,moussaileb_ransomwares_2018}. A decoy file is a dummy file, typically hidden from the user and created for ransomware detection. As no application is expected to use a decoy file, accesses to it are a strong signal of ransomware activity. 
Recently, Ganfure et al.~\cite{10026355} presented RTrap, an advanced version of traditional decoy files. 

Rtrap is a machine learning-based approach to decoy files to provide early detection against cryptographic ransomware. In particular, they propose a system to select a set of legitimate user files from the system, which are duplicated and deployed throughout the systems. The user files to be used as decoys are selected in such a way that they are representative of the user content on the machine. The insight behind the approach is that modern ransomware does not simply encrypt all files indiscriminately, but rather prioritizes certain types of file contents over others in order to be more effective. 
\textit{GonnaCharge}~\cite{panzade2024vig} showed that RTrap can be evaded by not trying to encrypt the user files in a particular directory at the very beginning but rather, stealthily  ﬁnd out which files can potentially be a decoy and then build an encryption plan out of it.

GonnaCharge, uses an initial recon phase that actually monitors events in the file system, i.e., file modifications, gathers this information and then processes it using machine learning techniques to detect possible decoy files set by RTrap and thus ignore them once it starts encrypting. In the same work, Panzade. et~al introduced Vig-War that essentially addresses the limitations of RTrap framework, mitigating GonnaCharge. 

Vig-War still employs decoy files to detect the ransomware activity by monitoring changes, renames, creations, and deletions of files similar to RTrap. On top of that it complements it by adding an extra layer of monitoring called iNode-watcher. iNodes serve as references or pointers to locate and access file data efficiently, utility that was utilized by GonnaCharge to evade RTrap. iNode watcher which monitors and tracks the access to iNodes of ﬁles and directories. Any unauthorized access to these iNodes will trigger an alert, indicating potential ransomware activity. If such activity is detected, then iNode watcher triggers necessary defensive actions to mitigate the attack.


More in general, many approaches exist that perform static analysis to identify ransomware~\cite{rezaei_pe_2021,zhu_few-shot_2022}, and malware~\cite{shalaginov_machine_2018}. All these works are orthogonal to our proposal and can be used together with \name to improve resilience.

In~\cite{de_gaspari_evading_2022}, the authors describe a family of evasion attacks against existing ransomware detectors. These attacks are discussed in Section~\ref{sec:EvasionAttack}. 
A high-level discussion of similar approaches to evasion was also addressed by \c{G}enc et al.~\cite{genc_next_2018}.
MalWASH~\cite{malwash}, D-TIME~\cite{dtime}, and ROPE~\cite{delia_rope_2021} are generic malware obfuscators that also leverage the distribution of malware workload across processes, similarly to~\cite{de_gaspari_evading_2022}. Rather than distributing malware workload, other approaches attempt to perturb the sequence of system calls generated by ransomware~\cite{rosenberg_query-efficient_2018,hu_black-box_2017}. 


As \name uses file-based behavioral profiles to detect malicious activity, it is resilient to these evasion attacks by design, regardless of the approach used to distribute malware behavior between processes.

Evasion techniques deployed in the wild commonly target detectors based on static features, which are relatively easy to evade. Examples of such evasion techniques include the use of obfuscation~\cite{saidi2010experiences} and packers~\cite{ugarte-pedrero_sok:_2015}, and memory-only malware~\cite{sudhakar_emerging_2020}. Many academic approaches exploit various adversarial ML techniques to guide mutation to various static features~\cite{grosse_adversarial_2017,rosenberg_generic_2018}. The detection technique discussed in this paper is based on dynamic behavior and, therefore, robust to static obfuscation.

Furthermore, in contrast to prior work on ransomware detection, \name was designed with the goal of being resilient to evasion attacks. This goal led to a detailed investigation of ransomware activity from which we decided to monitor and model the behaviour of the system activity from a file point-of-view given that prior work that relied on process-behaviour modeling was shown to be susceptible to evasion. On top of that, the features that were selected for monitoring were chosen following a push-pull paradigm, meaning that the alternation of one or more features would inevitably alter the rest of the remaining features thus leaving little to no room for evasive ransomware to try to evade detection. To evaluate this design choice, we actually performed various adaptive evasive attack attempts to evade \name detector, each of which resulted unsuccessful. To the best of our knowledge, we are the first to actually fully evaluate a ransomware detection approach from an adaptive adversary's point-of-view, feat that was not done in prior ransomware detection approaches.
